Contextual Expressive Text-to-Speech

The goal of expressive Text-to-speech (TTS) is to synthesize natural speech with desired content, prosody, emotion, or timbre, in high expressiveness. Most of previous studies attempt to generate speech from given labels of styles and emotions, which over-simplifies the problem by classifying styles and emotions into a fixed number of pre-defined categories. In this paper, we introduce a new task setting, Contextual TTS (CTTS). The main idea of CTTS is that how a person speaks depends on the particular context she is in, where the context can typically be represented as text. Thus, in the CTTS task, we propose to utilize such context to guide the speech synthesis process instead of relying on explicit labels of styles and emotions. To achieve this task, we construct a synthetic dataset and develop an effective framework. Experiments show that our framework can generate high-quality expressive speech based on the given context both in synthetic datasets and real-world scenarios.

==> misc/commands.tex <==
%!TEX root = ../main.tex

\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{epsfig}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{paralist}
\usepackage{enumerate}
%\usepackage{bm}
%\usepackage{enumitem}
%\usepackage[table]{xcolor}
%\usepackage[all]{xy}
\usepackage[color,matrix,arrow,all]{xy}
%\usepackage{cite}
\usepackage{comment}
\usepackage{booktabs}
\usepackage{balance}
\usepackage{stmaryrd}
\usepackage{pifont}
\usepackage{hhline}
%\usepackage{mathabx}
\usepackage{listings}
\usepackage{array}
\usepackage{float}
\usepackage[flushleft]{threeparttable}

\usepackage{mathrsfs}
\usepackage{makecell}
\usepackage{xparse}
\usepackage{wrapfig}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT DELETE!!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{tikz}
%\usetikzlibrary{trees}

\usepackage{epsfig}
\usepackage{multirow}
\usepackage{url}

\usepackage{multirow}
\usepackage{natbib}
\usepackage{graphicx}

%\usepackage{bm}
%\usepackage{amsfonts,amssymb}

\usepackage{listings}
\usepackage{framed}
\usepackage{xcolor}
\usepackage{color}
\usepackage{geometry}
\usepackage{changepage}


\newcommand{\red}[1]{\textcolor{red}{#1}}
\definecolor{green}{RGB}{0,128,0}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\definecolor{yellow}{RGB}{255,200,18}
\newcommand{\yellow}[1]{\textcolor{yellow}{#1}}
\newcommand{\pink}[1]{\textcolor{magenta}{#1}}

\newcommand{\add}[1]{\textcolor{blue}{{#1}}}
% \newcommand{\add}[1]{\textcolor{black}{{#1}}}
\newcommand{\addd}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\rewrite}[1]{\textcolor{gray}{{#1}}}
\newcommand{\notice}[1]{\textcolor{red}{{#1}}}



\newcommand{\ie}{{\em i.e.,}\xspace}
\newcommand{\eg}{{\em e.g.,}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\aka}{\emph{a.k.a.}\xspace}
\newcommand{\kwlog}{\emph{w.l.o.g.}\xspace}

\newcommand{\eop}{\hspace*{\fill}\mbox{$\Box$}}     % End of proof


==> sec/framework_changedata.tex <==
\section{The Framework of FTTS}
\label{sec:framework}

The proposed FTTS extracts the emotional, contextual, personal information from generalized free text and generates speech with corresponding prosody, timbre, tone and style. 
In the following subsections, we first introduce the dataset we reorganized for this task in Section \ref{subsec:data_construct}. Then, we describe our model FTTS in detail. AS shown in Figure~\ref{fig:fr},  FTTS is a encoder-decoder based model. The encoder models the interaction of controlling text and context text in Section \ref{subsec:text_encoder}. The decoder generates speech autoregressively in Section \ref{subsec:audio_decoder}. Finally, we introduce the training process of FTTS in Section \ref{subsec:training_process}.

\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/frame2.pdf}
%   \caption{The framework of FTTS, which consists of three modules: Text Controlled Encoder, Attention-based Auto-Regressive Audio
% Decoder and a well pretrained vocoder. }
  \caption{The framework of FTTS, which consists of four modules: free text speech data preprocess, text controlled encoder, attention-based auto-regressive speech
decoder and a well pretrained vocoder. }
\label{fig:fr}
 % \vspace{-1em}
\end{figure}

\subsection{Free Text Speech Dataset}
\label{subsec:data_construct}

To get both the text understanding and speech generation abilities for FTTS, we reorganize a free text speech dataset. By merge open-source labeled speech datasets and emotional text datasets. Each sample of the free text speech dataset consists of controlling free text, content text and the speech.

We use emotional labels to merge these datasets together. As shown in Figure \ref{fig:fr}, common labeled expressive speech datasets contain labels of emotion, speaker name, content text, etc, while common emotional text datasets have text samples and their emotional labels. For a sample in labeled speech datasets, we randomly select a sample with similar emotional label in emotional text datasets. The controlling free text is the combination of text in emotional text datasets and other labels in labeled speech datasets by a template. For example in Figure \ref{fig:fr}, the free text is ``\textit{It’s a nice day. Bea said:}'', which is combined by ``\textit{It’s a nice day}'' in emotional text dataset and the speaker name ``\textit{Bea}'' in labeled speech dataset. 
The content text and the speech are the same as labeled speech dataset.





%



\subsubsection{Datasets}
\label{subsec:dataset}





% We use Emotional Voices Database (EmoV-DB)~\cite{adigwe2018emotional} and Yelp Review Dataset (Yelp)~\cite{li2018delete}. EmoV-DB is a widely used emotional voice dataset that reads transcripts from the CMU Arctic Database~\cite{kominek2004cmu}. For each transcript, EmoV-DB contains voices of five emotions from four speakers (two male and two female). 
% Yelp is a natural language text dataset with obvious emotions, including texts of positive emotions and negative emotions.
% %
% We use EmoV-DB and Yelp to build a Free-Text-Controlled TTS (FTTS) dataset. In detail, as shown in Table~\ref{tbl:data}, for each text-speech pair with amused or angry emotions, we randomly select three corresponding positive or negative texts from yelp as contexts to form three different FTTS data items. Overall, we create a Free-Text-Controlled TTS dataset with 5912 data items, which contains four speakers and two emotions for training and evaluation our model.
% Like study~\cite{kreuk2021textless}, we generate train/valid/test sets with the ratio of 90/5/5, and report the performance on test set.
The training dataset is formed as is described in Section \ref{subsec:data_construct}. 
We use Emotional Voices Database (EmoV-DB)~\cite{adigwe2018emotional} as the labeled speech dataset and Yelp Review Dataset (Yelp)~\cite{li2018delete} as the emotional text dataset.
EmoV-DB is a widely used emotional voice dataset that reads transcripts from the CMU Arctic Database~\cite{kominek2004cmu}. For each transcript, EmoV-DB contains voices of five emotions from four speakers (two male and two female).
Yelp is a natural language text dataset with obvious emotions, including texts of positive emotions and negative emotions. 
Table~\ref{tbl:data} present some samples of the reorganized free text speech dataset.
For each text-speech pair with amused or angry emotions, we randomly select three corresponding positive or negative texts from yelp as controlling text to form three different  data samples. Overall, we create a free text speech dataset with 5912 data samples, which contains four speakers and two emotions for training and evaluation our model.
Like study~\cite{kreuk2021textless}, we generate train/valid/test sets with the ratio of 90/5/5, and report the performance on test set.
We also use a larger speech dataset LJSpeech~\cite{ljspeech17} for pre-training a TTS model that without context, because the emotional speech and context are limited.



==> sec/intro.tex <==
\section{Introduction}
\label{sec:intro}

Text-to-speech (TTS) is the task of generating speech from input text, which is useful for a large number of practical problems, such as machine reading, human-computer interaction, etc. 
%
Compared with TTS, expressive TTS requires more emotional speech, which has various prosodies rather than neutral speech (\ie narrative speech) that has monotonic prosody. 

With the success of the generation model based on deep learning, end-to-end TTS model~\cite{wang2017tacotron,ping2017deep,tachibana2018efficiently} that input text (\eg character, phone, etc.) has been able to generate high-quality and natural speech (wav, etc.).
%
Expressive TTS needs to consider integrating prosodic features into speech generation. 
At present, the mainstream method is to use a condition vector that represents emotion, speaker, or other signals to control the speech generation. The construction methods of condition vector contain manual definition or dynamic learning during TTS training, and the latter is the most commonly used in end-to-end expressive TTS model~\cite{gibiansky2017deep, lee2017emotional, henter2017principles}. 
%
One kind of learned condition vector comes from the displayed labels~\cite{gibiansky2017deep, lee2017emotional}, for example, given an emotion label, and learning the emotion embedding in the training process, and integrating it into speech generation.
%
Another way for learning condition vector is to learn implicit controlled embedding from reference speech~\cite{lei2022msemotts,skerry2018towards,wang2018style}. That is, instead of specifying a specific controlled label, it inherits the characteristics in the reference speech.

The above settings are lack of practicality and difficult to obtain training data. On one hand, in real scenes, it is difficult to classify the emotion, prosody, personality of speech with specific labels; On the other hand, there are few expressive speech datasets with accurate labels or appropriate reference speeches, and the cost of obtaining these expressive datasets is high. Therefore,  we introduce a new task setting for expressive TTS, i.e., \textbf{semantic context controlled TTS}, which means learning the corresponding emotion, personality and  condition information directly from the contextual text and using it to control the speech generation.

To achieve the semantic context controlled TTS task, 
we propose a new framework named as CTTS, which uses semantic context as context to guide speech generation. CTTS aims to model the personality, emotion and other information of the context to guide the generation of reasonable and expressive speech. 
Obviously, CTTS has high practical value, such as audio book in accordance with the context, or an expressive voice assistant. 
% Meanwhile, training data for CTTS is easy to obtain, while massive public emotional texts can be used directly.

The challenges faced by CTTS are mainly text understanding and speech generation. Fortunately, current multimodal pre-training model can well understand multiple modalities such as text, image and speech at the same time. Therefore, we design an effective framework for CTTS. 
In CTTS, we first reorganize a synthetic dataset for this task. Then, we design an encoder-decoder TTS model for speech generation. Experiments show that, although our model is trained on a synthetic dataset, it still could perform well in zeroshot real-world settings.

% The model consists of four parts: \textbf{Data preprocessing} gets data embeddings for free text and speech content text; \textbf{Encoder} extracts hidden embedding that containing all text semantics; \textbf{Decoder} generates speech features Mel-spectrum; \textbf{Vocoder} converts Mel-spectrum into speech.

% free text speech data preprocess, text controlled encoder, attention-based auto-regressive speech decoder and a well pretrained vocoder.

Our notable contributions are summarized as follows:
\begin{itemize}
% \item  We propose a new Expressive TTS task, \textbf{Free-text-controlled TTS (CTTS)}, which using free text semantics to control speech emotion.
 \item To our knowledge, it is the first time using generalized semantic context to control expressive speech generation. 
% Meanwhile, we release a benchmark of the task, so that researchers and practitioners can directly use it. 
Meanwhile, we reorganize a new dataset for the task. 
\item We develop effective end-to-end framework \textbf{semantic context-controlled TTS (CTTS)} \footnote{Our code is based on OFA~\cite{wang2022unifying} and will be released here if the paper is accepted. }, which is simple and efficient, including data preprocessing, encoder, decoder and vocoder modules.
% \item We conduct a complete experiment to compare the effectiveness of our proposed method, and the speeches generated by our method CTTS can ensure the accuracy, naturalness and expressiveness of speech generation.
\item Experiments show that the speeches generated by CTTS can ensure the accuracy, naturalness and expressiveness of speech generation both in synthetic and zeroshot real-world settings..
\end{itemize}





==> sec/rw.tex <==
\section{Related Work}
\label{sec:rw}

\textbf{Text-to-Speech (TTS)}: ...

\textbf{Emotional TTS}: ...






